DeFMO: Deblurring and Shape Recovery of Fast Moving Objects

Objects moving at high speed appear significantly blurred when captured with cameras. The blurry appearance is especially ambiguous when the object has complex shape or texture. In such cases, classical methods, or even humans, are unable to recover the object's appearance and motion. We propose a method that, given a single image with its estimated background, outputs the object's appearance and position in a series of sub-frames as if captured by a high-speed camera (i.e. temporal super-resolution). The proposed generative model embeds an image of the blurred object into a latent space representation, disentangles the background, and renders the sharp appearance. Inspired by the image formation model, we design novel self-supervised loss function terms that boost performance and show good generalization capabilities. The proposed DeFMO method is trained on a complex synthetic dataset, yet it performs well on real-world data from several datasets. DeFMO outperforms the state of the art and generates high-quality temporal super-resolution frames.

==> tables/datasets.tex <==
\newcommand{\addtypimg}[1]{ \raisebox{-0.15em}{\multirow{3}{*}{\includegraphics[width=0.11\linewidth]{imgs/typical/#1}} }}

\begin{table*}[t]
\centering
\small
\newcommand{\CNameFA}[1]{ \raisebox{0.1em}{\multirow{ 3}{*}{\rotatebox[origin=l]{90}{\scriptsize #1 }}} }
\newcommand{\CName}[1]{ {\footnotesize #1 } }
\setlength{\tabcolsep}{2.1mm} % width
\renewcommand{\arraystretch}{1.2} % height
\begin{center}
\begin{tabular}{@{}c@{\hskip 0.2em}c@{}rcccccccc@{}}

% \toprule
\specialrule{.1em}{.05em}{.05em} 

 \multirow{2}{*}[-5pt]{\rotatebox[origin=l]{90}{\footnotesize Dataset}} & \multirow{2}{*}{\CName{Typical Object}} & \multirow{2}{*}{\CName{Score}} & \multicolumn{2}{c}{ \CName{Inputs} } & \multicolumn{4}{c}{  \CName{Compared Methods} }  &  \CName{Proposed} &  \CName{Traj. Oracle} \\
  \cmidrule(lr){4-5} \cmidrule(lr){6-9} \cmidrule(lr){10-10} \cmidrule(lr){11-11}

 &  &  & \CName{$B$} & \CName{$I$} & \CName{Jin~\etal~\cite{Jin_2018_CVPR}} & \CName{Debl.GAN~\cite{Kupyn_2019_ICCV}} & \CName{TbD~\cite{tbd}} & \CName{TbD-3D~\cite{tbd3d}} & \CName{DeFMO} & \CName{TbD-3D-Or.}  \\ 
 
 \hline

 \CNameFA{Falling~\cite{kotera2020}} & \addtypimg{falling} & TIoU$\uparrow$ & N/A & N/A & N/A & N/A & 0.545 & 0.545 & \winner{0.703}  & 1.000 \\
 
 & & PSNR$\uparrow$ & 19.68 & 23.73 & 23.54 & 23.36 & 22.09 & 23.01  & \winner{26.80} & 22.82 \\
  
 & & SSIM$\uparrow$ & 0.459 & 0.593 & 0.575 & 0.588 & 0.617 & 0.695 & \winner{0.752} & 0.701  \\

\hline

 %%%%%%%%%%%%% tbd3d
\CNameFA{TbD-3D~\cite{tbd3d}} & \addtypimg{tbd3d} &  TIoU$\uparrow$ & N/A & N/A & N/A & N/A  & 0.539 & 0.539  & \winner{0.850} & 1.000 \\

 & & PSNR$\uparrow$ & 19.81 & 24.80 & 24.52 & 23.58  & 19.67 & 21.99 & \winner{26.23} & 24.63  \\
  
 & & SSIM$\uparrow$ & 0.425 & 0.640 & 0.590 & 0.603 & 0.483 & 0.621 &  \winner{0.699} & \oracle{0.703}  \\

\hline
 %%%% tbd3d end  

  %%%%%%%%%%%%% tbd 
\CNameFA{TbD~\cite{tbd}} & \addtypimg{tbd} &  TIoU$\uparrow$ & N/A & N/A & N/A & N/A  & \winner{0.601} & \winner{0.601}  & 0.583 & 1.000 \\

 & & PSNR$\uparrow$ & 21.51 & 25.07 & 24.90  & 24.27  & 23.99 & 24.57  & \winner{25.54} &  \oracle{26.23}  \\

 & & SSIM$\uparrow$ & 0.467 & 0.569 & 0.530 & 0.537 & 0.612  & \winner{0.678} &  0.599 &  \oracle{0.712} \\
 \hline 
 %%%% tbd end 


\multicolumn{3}{c}{Runtime (on $240 \times 320$)} & N/A & N/A & 2 fps & 10 fps & 0.01 fps & 0.001 fps  & \winner{20 fps} & 0.001 fps \\

% \bottomrule
\specialrule{.1em}{.05em}{.05em} 

\end{tabular}
\end{center}
\vspace{-0.8em}
\caption[Something]{\textbf{Evaluation on:} Falling Objects~\cite{kotera2020}, TbD-3D~\cite{tbd3d}, TbD~\cite{tbd} datasets\footnotemark. 
% The Falling Objects dataset is the most challenging one, as it contains 6 sequences with fast moving objects of arbitrary shapes and textures,~\eg key, pen, marker, \etc. The TbD-3D dataset contains only sports sequences with mostly spherical but significantly textured objects. The TbD dataset is the simplest one, with mostly spherical and uniformly colored objects.
The datasets are sorted by decreasing difficulty: arbitrary shaped and textured~\cite{kotera2020}, mostly spherical but significantly textured~\cite{tbd3d}, and mostly spherical and uniformly colored objects~\cite{tbd}.
DeFMO is superior to the compared methods by a wide margin on all datasets except for the easiest~\cite{tbd} since the TbD(-3D) methods~\cite{tbd,tbd3d} are specifically designed for such easy cases. TbD-3D-Oracle~\cite{tbd3d} is given ground truth trajectories and estimates only sub-frame appearance. }
\label{tbl:datasets}
\end{table*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{tabular}{clcccccccc}

% \specialrule{.1em}{.05em}{.05em}

%  \CName{Set} & \CName{Score} & \CName{Background} & \CName{No deblur} & \CName{Jin~\etal~\cite{Jin_2018_CVPR}} & \CName{DeblurGAN-v2~\cite{Kupyn_2019_ICCV}} & \CName{TbD~\cite{tbd}} & \CName{TbD-3D~\cite{tbd3d}} & \CName{TbD-3D-Oracle} & \CName{DeFMO (ours)}  \\ \hline
 
%  \CNameFA{\cite{kotera2020}} & TIoU & N/A & N/A & N/A & N/A & 0.545 & 0.545 & N/A & \winner{0.703} \\
 
%  & PSNR & 19.680 & 23.728 & 23.540 & 23.358 & 22.091 & 23.009 & 22.820 & \winner{26.382}  \\
  
%  & SSIM & 0.459 & 0.593 & 0.575 & 0.588 & 0.617 & 0.695 & 0.701 & \winner{0.750}  \\
                
%  %%%%%%%%%%%%% tbd3d
%  \hline 
%  \CNameFA{\cite{tbd3d}} & TIoU & N/A & N/A & N/A & N/A  & 0.539 & 0.539 & N/A & \winner{0.850} \\

%  & PSNR & 19.808 & 24.796 & 24.515 & 23.579  & 19.665 & 21.985 & 24.625 & \winner{26.023}  \\
  
%  & SSIM & 0.425 & 0.640 & 0.590 & 0.603 & 0.483 & 0.621 & \winner{0.703} &  0.694  \\
                
%  \hline 

%  & Runtime & N/A & N/A & \winner{20 fps} & 15 fps & 0.5 fps & 0.1 fps & 0.1 fps & \winner{20 fps} \\
%  %%%% tbd3d end

% \specialrule{.1em}{.05em}{.05em}

% \end{tabular}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Evaluation on falling objects dataset~\cite{kotera2020} which contains 6 sequences with fast moving objects~--~key, box, eraser, pen, cell, marker. DeFMO method is superior to other baselines by a wide margin. The second best performing method is TbD-3D-Oracle~\cite{tbd3d}, which is provided with ground-truth trajectories and estimates only sub-frame appearances.

%%%%%%%%%%%
% AVERAGES
% DeFMO: tiou 0.689, psnr 26.109 dB, ssim 0.747
% DeFMO: time 0.098 seconds
% Imr: psnr 23.728 dB, ssim 0.593
% Bgr: psnr 19.680 dB, ssim 0.459
% tbd: tiou 0.545, psnr 22.091 dB, ssim 0.617
% tbd3d: tiou nan, psnr 23.009 dB, ssim 0.695
% tbd3d: time 253.790 seconds


==> tables/tbd.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{2mm} % width
% \renewcommand{\arraystretch}{1.2} % height
\begin{center}
\begin{tabular}{@{}lccccc@{}}

\toprule

 Score & Background & No deblur & TbD~\cite{tbd} & DeFMO  \\ \midrule

 TIoU & N/A & N/A & \winner{0.601} & 0.490 \\
 PSNR &  22.839 & 25.370   & 24.976 & \winner{25.152}  \\
  
 SSIM & 0.426 &  0.498   & \winner{0.636} &  0.573 \\

\bottomrule

\end{tabular}
\end{center}
\vspace{-0.5em}
\caption{Evaluation on the TbD dataset~\cite{tbd}, compared to the TbD method. DeFMO method is inferior to TbD in the setting when the fast moving object does not change its appearance within one frame and has a trivial shape (mostly spherical here).  }
\label{tbl:tbd}
\end{table}

% oracle: 27.255 dB, ssim 0.725

==> tables/tbd3d.tex <==
\begin{table*}[t]
\centering
\setlength{\tabcolsep}{4mm} % width
% \renewcommand{\arraystretch}{1.2} % height
\begin{center}
\begin{tabular}{lcccccc}

\specialrule{.1em}{.05em}{.05em}

 Score & Background & No deblur & TbD~\cite{tbd} & TbD-3D~\cite{tbd3d} & TbD-3D-Oracle & DeFMO (ours)  \\ \hline

 TIoU & N/A & N/A & 0.539 & 0.539 & N/A & \winner{0.850} \\

 PSNR & 19.808 & 24.796  & 19.665 & 21.985 & 24.625 & \winner{26.023}  \\
  
 SSIM & 0.425 & 0.640  & 0.483 & 0.621 & \winner{0.703} &  0.694  \\
                
 \hline 

Runtime & N/A & N/A & 0.5 fps & 0.1 fps & 0.1 fps & \winner{20 fps} \\

\specialrule{.1em}{.05em}{.05em}

\end{tabular}
\end{center}
\caption{Evaluation on the TbD-3D dataset~\cite{tbd3d}. For all scores, higher value means better result. The proposed DeFMO method outperforms other baselines. TbD-3D-Oracle is slightly better in terms of SSIM but the difference is negligible, considering that TbD-3D-Oracle is provided with the ground truth trajectories. }
\label{tbl:tbd3d}
\end{table*}

% 0.447

% Jin et al 24.515 dB, ssim 0.590
